Making I/O Virtualization Easy with Device Files

Personal computers have diverse and fast-evolving I/O devices, making their I/O virtualization different from that of servers and data centers. In this paper, we present our recent endeavors in simplifying I/O virtualization for personal computers. Our key insight is that many operating systems, including Unix-like ones, abstract I/O devices as device files. There is a small and stable set of operations on device files, therefore, I/O virtualization at the device file boundary requires a one-time effort to support various I/O devices. We present devirtualization, our design of I/O virtualization at the device file boundary and its implementation for Linux/x86 systems. We are able to virtualize various GPUs, input devices, cameras, and audio devices with fewer than 4900 LoC, of which only about 300 are specific to I/O device classes. Our measurements show that devirtualized devices achieve interactive performance indistinguishable from native ones by human users, even when running 3D HD games.

==> architecture.tex <==
\section{Architecture Support}
\label{sec:architecture_support}

Storyline of this section: We currently use shadow page table to support
the hybrid address space. But TDP (e.g., Intel EPT and AMD NPT) are the
future of memory virtualization as they have much better performance
than shadow page tables. Their improved memory performance can indeed
help the memory-mapped I/O performance of devirtualization. However, we
cannot use TDP to create shadow page tables. According to Sri, this is
because the TDP is only enabled in the user mode. In this section, we
can discuss how TDP can be modified to support devirtualization. We
should also try to mention how the added architecture support can
benefit other scenarios too in addition to devirtualization.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> udd_design.tex <==
\section{Design of Universal Virtual Driver (UVD)}

In this section, we provide details regarding the design of the
universal virtual driver (UVD). The same design applies to all I/O
devices although for each devirtualized I/O device, there will be
a dedicated UVD backend in the host and a dedicated UVD frontend in the
guest. In the guest, the UVD frontend appears to be the device driver,
receives file operations issued to the device, and forwards them to the
backend in the host. The backend feeds the file operations properly to
the device driver and return the results back to the frontend. The
frontend finally delivers the results to the guest process as if it were
the device driver.

The communication between the UVD frontend and backend is critical to
the performance of devirtualization. Therefore, we employ a careful
combination of hypercall, virtual registers~\footnote{aas: similar to my
comment in Section 2, I think we can just use hypercalls here. In
implementation, we mention that for x86 and KVM hypervisor, virtual
registers are used to pass arguments}, virtual interrupt and
virtual memory techniques to improve the communication efficiency. The
virtual memory technique, called \textit{hybrid address space}, obviates
bulk data exchange between the frontend and backend, and will be
discussed in Section~\ref{sec:hybrid_address_space} in detail. In this
section, we focus on file operation forwarding and
notification~\footnote{lz: may revise later}. 

\subsection{File Operation Forwarding}

The UVD frontend employs hypercalls and guest virtual registers to
forward file operations to the backend efficiently. The results from
a file operation are sent back to the frontend through either virtual
registers or the hybrid address space~\footnote{aas: how so through the
hybrid address space? If you mean shared memory pages, they are
different from hybrid address space}. 

Like that a system call is a software trap from a user space process to
the kernel, a \textit{hypercall} is a software trap from a guest
operating system to the hypervisor. The guest can use hypercalls to
request privileged services from the host. The guest stalls until the
hypercall returns~\footnote{aas: note to self: investigate and update}. When forwarding a file operation, the UVD frontend in
the guest pack the type and arguments of the file operation into virtual
registers and calls a hypercall. The UVD backend recovers the file
operation and its augments upon receiving this hypercall and deliver the
file operation to the device driver.  Similarly, just before returning
from the hypercall, the UVD backend puts the results of the operations on the guest
virtual registers, and the UVD frontend recovers the results~\footnote{lz:
whose arguments? file operation? or hypercall? {\bf revised}}.  

%We employs hyper calls
%because hypercalls are increasingly efficient on modern CPU's.  For
%example, Intel x86 architecture provides the {\tt VMCALL} instruction to
%implement the hypercall, and this instruction only takes a few hundreds
%CPU cycles [XXX]. 

Because the UVD backend is shared by all guests and their processes, it
must associate a forwarded file operation and its return to the right
guest and the right process. The backend identifies the guest with
information from the hypervisor, which knows the virtual CPU that
generated the hypercall, and hence knows the guest.~\footnote{lz: where is this information kept by the
hypervisor? {\bf revised. When there is a hypercall, the hypervisor
looks at the execution status and figures out which virtual CPU
generated the hypercall. Knowing the virtual CPU, we know which guest
did it. However, I don't know more details of how the hypervisor figures
out the virtual CPU.}}. In order to identify the process, the UVD backend
leverages a particular virtual register of the identified guest; this
virtual register, e.g., {\tt CR3} in x86, holds a pointer to the shadow
page table of the process that issued the file operation and therefore yielded
the control the guet kernel~\footnote{lz: is this page table for the process that
issued the file operation and therefore yielded control to the guest
OS? {\bf revised. I also understand that it might sound confusing that
the guest virtual register has a pointer to the shadow page table. THe
hypervisor plants in this register}}. The UVD backend can use this pointer value to distinguish between
different guest process shadow page tables, and hence between different
processes~\footnote{lz: I understand that using this register, you can
tell a file operation is from a unique process and two file operations
are from different processes. What is not clear to me is how the backend
can deliver the results back to the process. I actually understand that
for synchronous UVD, this is not a problem because the guest stalls. For
asynchronous UVD, how will it be soved? {\bf I haven't done this, but
I guess it can be done by using some operation tag. That is, each
operation gets a number tag and the backend can send the results to the
frontend using that tag, and the frontend knows which tags belongs to
which processes}} .

%{\bf Virtual Interrupt}: The UVD backend can initialize a communication
%with the UVD frontend using virtual interrupts. Devirtualization uses
%virtual interrupts only for notifications (Section XXX). Injecting
%a virtual interrupt into the guest is a relatively expensive operation.
%In Section XXX, we present measurements on its overhead.

%{\bf Shared Memory Pages}: Shared memory pages provide another mechanism
%for communication between the UVD frontend and backend. A shared memory
%page is a physical memory page that is mapped at the same virtual
%address in both the host and the guest. Therefore, any writes to the
%virtual addresses of this page by either end of UVD will be immediately
%visible to the other end. Shared memory pages can be used instead of the
%virtual iterrupt, since virtual interrupts have high overhead. Note that
%just a few shared pages are enough for the UVD communication, because as
%it was mentioned above, the UVD communication is minimal.

\subsection{Notifications}
\label{sec:asynchronous}

~\footnote{lz: please replace VFS with device file in the figures. Please explain how the UVD tracks which processes to deliver the signal. Please read the previous subsection first. I don't feel the two figures are necessary for understanding. }

As explained in Section~\ref{sec:device_files}, processes can request for notifications for
new events generated by a device. Notifications pose a unique challenge
for devirtualization as host device drivers need to notify the guest
processes of new events. In our solution, UVD backend receives the
notification signals in the host and injects them as virtual interrupts
into the guest, and UVD frontend then signals the guest processes. 

\begin{comment}
Figure~\ref{fig:async_notif_1} demonstrates how notifications works in
Linux: processes issue a file operation to
announce that they are interested in events generated by a device.
This operation is handed to the device driver, which adds the process ID to the list of the processes
that are waiting for events from a device. Whenever there is a new
event, the device driver sends signal ({\tt SIGIO} in Linux) to all the processes
that waiting for this new event. Once a process receives the signal, it
reads the
new event by issuing a read operation on the device file. In Linux, the
signal does not identify which device generated the event. Therefore, if
the process is waiting for events from multiple devices, e.g., mouse and
keyboard, it has to first poll all of using the poll file operation
before read.
\end{comment}

%Figure~\ref{fig:async_notif_2} shows how notifications work in
%devirtualization: 

When a process requests for notifications from a devirtualized device,
the request operation is handed to the UVD frontend. The UVD frontend
then adds the process ID to the list of waiting processes. Whenever new
events are generated, the host VFS informs the UVD backend. The UVD
backend then informs the UVD frontend with a virtual interrupt.  The
virtual interrupt is on a special interrupt line that is reserved and
handled by the UVD frontend. The UVD frontend then sends a signal to the
guest processes in the list. The UVD frontend maintains different lists
for processes are waiting for events from different devices, and therefore,
the UVD backend informs the UVD frontend of which device generated the
event by sending virtual interrupts on a different interrupt line for
each device. 

%\begin{comment}
%Using interrupts to deliver the signal to the guest incurs noticeable
%latency, as will be demonstrated in Section XXX. While this latency is
%much smaller than the minimum requirement for input devices, it might
%become a bottleneck for other performance-sensitive I/O devices, such as
%network devices. One alternative design to reduce this latency is using
%shared memory pages between the host and the guest. That is, upon
%receiving a host signal, the UVD backend can mark some flag in the
%shared page to notify the UVD frontend of the signal. {\bf aas we need
%to think more about this. Sri told me that this solution can be made to
%be much faster than interrupts}
%\end{comment}



